Qualitative Approximate Behavior Composition

The behavior composition problem involves automatically building a controller that is able to realize a desired, but unavailable, target system (e.g., a house surveillance) by suitably coordinating a set of available components (e.g., video cameras, blinds, lamps, a vacuum cleaner, phones, etc.) Previous work has almost exclusively aimed at bringing about the desired component in its totality, which is highly unsatisfactory for unsolvable problems. In this work, we develop an approach for approximate behavior composition without departing from the classical setting, thus making the problem applicable to a much wider range of cases. Based on the notion of simulation, we characterize what a maximal controller and the "closest" implementable target module (optimal approximation) are, and show how these can be computed using ATL model checking technology for a special case. We show the uniqueness of optimal approximations, and prove their soundness and completeness with respect to their imported controllers.

==> 5-Solution.tex <==
\section{Computing Optimal Target Approximations}\label{sec:solution}
%\newcommand{\OptApprox}{\mbox{\textit{OptApprox}}}
\newcommand{\OptApprox}{{\textsf{\small ComputeApprox}}}
\newcommand{\INDSTATE}[1][1]{\STATE\hspace{#1\algorithmicindent}}

%\begin{itemize}
%\item Graph from combining enacted system and target.
%\item Target extraction.
%\item Checking for solution. Theorem - Unique maximal approximation. Discuss why adding a $nop$ to maximal approximation with ``dead ends'' is not a solution though maximal simulation.
%\item Target reduction by using bisimulation quotient (used in model checking). DFA minimization cannot be used here.
%\item Complexity
%\end{itemize}


Let us now explain how to effectively construct an optimal approximation of a given target on an available system.
%%
% The technique involves constructing a maximal sub-part of the target module such that composition exactness can be recovered.
% %%
The central idea involves eliminating (target) transitions that could potentially lead the system to dead-ends, states where no further action requests can be honoured. 


Algorithm~\ref{algo:optimalTargetApprox} takes an available system and a target behavior, and returns an optimal approximation of the target. 
%%
To that end, it works on the so-called \emph{full enacted system behavior}, the transition system that represents the joint evolution of the target module with the available system.
%%
Technically, the full system behavior is the synchronous product between the target and the enacted system.
%%
Given a system $\S$ with enacted system $\E_\S=\tup{S_{\S},\A_\S, \set{1,\ldots,n},s_{\S0},\delta_\S}$ and a target behavior $\T=\tup{T,\A,t_0,\varrho_T}$, the \defterm{full enacted system behavior} of $\tup{\S,\T}$ is a tuple $\E_{\tup{\S,\T}}=\tup{S_{\F},\A, \{1,\ldots,n\},s_{\F0},\delta_\F}$, where:
%
\begin{itemize}
\item $S_\F =  S_\S \times T$ is the finite set of $\E_{\tup{\S,\T}}$'s states;  when $s_\F=\tup{s_\S, t}$, we denote $s_\S$ by $\sys(s_\F)$ and $t$ by $\tgt(s_\F)$;
% 
\item $s_{\F0}\in S_\F$, with $\sys(s_\F)=s_{\S0}$ and $\tgt(s_{\F0}) = t_0$, is $\E_{\tup{\S,\T}}$'s initial
  state;
%
\item $\delta_\F\subseteq S_\F \times \A \times \{1,\ldots,n\} \times S_\F$ is   $\E_{\tup{\S,\T}}$'s transition relation, where  $\tup{s_\F,a,k,s_\F'} \in  \delta_\F$, or $s_\F \goto{a,k}  s_\F'$ in $\E_{\tup{\S,\T}}$ \emph{iff}
\begin{itemize}
\item $\tgt(s_\F)\goto{a}\tgt(s_\F')$ in $\T$; and
\item  $\sys(s_\F)\goto{a,k} \sys(s_\F')$ in $\E_\S$.
\end{itemize}
\end{itemize}


Transitions in $\E_{\tup{\S,\T}}$ are such that the action involved can be performed by both the enacted system (i.e., some available behavior) as well the target module. 
%%
As a result, those target actions that cannot be matched by the system are excluded from the full system behavior and, therefore, it may have states with no outgoing transitions, that is, dead-ends.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% OTA ALGORITHM  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Algo_ota} 


% 
% \begin{figure*}[!t] 
% \begin{center}
% \resizebox{!}{.75\columnwidth}{
% \input{Algo-example}
% }
% \caption{A part of the full enacted system behavior for the smart house scenario (with target $\TEX$). Since, in this part, audio behavior $\B_A$ is always at initial state $b_0$, it is not included explicitly. Dashed components will be removed by the algorithm.}
% \label{fig:ambientIntel-fullsystem}
% \end{center}
% \end{figure*}



The $\OptApprox$ algorithm basically extracts an (optimal) target approximation from the full enacted transition system by repetitively projecting out (i.e., deleting) states and transitions as follows.
%% 
In steps 3 and 4, all dead-end states with no outgoing transitions are removed from the (current) full enacted system. These represent states in which the whole system will be \emph{stuck}, as no target request can be fulfilled.
%%
Steps 5 and 6 are more involved, and amount to removing all ``moves" that may lead to one of the states just deleted. So, suppose a transition $\tup{s_\F,a,k,s_\F'}$ is removed from the (current) full enacted system, that is, the target is requesting transition $\tgt(s_\F) \goto{a} \tgt(s_\F')$ whose action $a$ has been delegated to available behavior $k$. Then, such transition was removed because that request-delegation pair may potentially lead---due to non-determinism in the system---to a state that has just been removed (in steps 3-4). Intuitively, that request-delegation step is a ``risky'' one, in that it could lead to an overall dead-end state.


Steps 3 to 6 are repeated until no further reduction can be achieved.
%%
Once that happens, a target behavior is obtained by merely projecting out the behavior delegation indexes in transitions (step 8). Finally, the so-called  \emph{bisimulation quotient} technique~\cite{ModelCheckingBaier:2008} is applied to the resulting target behavior (step 9), a useful notion used in model checking for state space reduction. 
%%
Technically, when $\B$ is a behavior and $\cong_{\B}$ is the largest bisimulation relation of $\B$ with itself, then $\B/{\cong_\B}$ is the so-called \emph{quotient transition system} of $\B$ under $\cong_{\B}$, and is such that $\B \cong \B/({\cong_\B})$~\cite{ModelCheckingBaier:2008} and typically substantially smaller than $\B$, by means of putting together bi-similar states. In the case of our  $\OptApprox$ algorithm, we have that $\aprxtgt \cong (\aprxtgt/{\cong_{\aprxtgt}})$.
% Technically, when $\B = \tup{B,\A,b_0,\varrho}$ is a behavior, $\cong_{\B}$ is the largest (bi)simulation relation of $\B$ with itself, the \defterm{quotient transition system} of $\B$ under $\cong_{\B}$, denoted $\B/{\cong_\B}$, is defined as the tuple $\B/{\cong_\B} = \tup{B', \A,[b_0]_{\cong_\B},\varrho_{\cong_\B}}$, where:
% %%
% \begin{itemize}
%   	\item $[b]_{\cong_\B} = \{ b' \in B \mid  b \cong_\B b' \}$, that is, $[b]_{\cong_\B}$ stands for the \emph{equivalence class} of state $b$ w.r.t. $\cong_\B$ (all states in $\B$ which are in bi-simulation with $b$); 
% 
% 	\item $B' = \{ [b]_{\cong_\B} \mid b \in B \}$ is the \emph{quotient space}, the set of equivalent classes in $B$ w.r.t. $\cong_\B$; and  
% 
%   \item $\tup{[b]_{\Sim_\B},a,[b']_{\cong_\B}} \in \varrho_{\cong_\B}$ \emph{iff} $\tup{b,a,b'} \in \varrho$.
% \end{itemize}
% 
% \noindent
% That is, the bisimulation quotient attains a state space reductions leading to more compact approximations by putting together states that are in bisimulation.
% %%
% It follows then that $\B \cong \B/({\cong_\B})$~\cite{ModelCheckingBaier:2008}, and in the case of our  $\OptApprox$ algorithm, $\aprxtgt \cong (\aprxtgt/{\cong_{\aprxtgt}})$ follows.
%  
%


% \begin{example}
% Figure~\ref{fig:ambientIntel-fullsystem} shows part of the full enacted system for the smart house scenario.
% %
% Initially only action $\aLightOn$ can be performed, by delegating it to the light device $\B_L$, thus evolving such behavior and the target module $\TEX$.
% %
% Observe how, after that, $\aMovie$ action can be delegated to two different devices, namely, the movie device $\B_M$ or the game device $\B_G$. (State $s_1$ will also be able to transition on action $\aMusic$ but that is not shown in the figure.)
% %
% Importantly, depending on which available behavior is selected, the target's transition requests that could be honoured next differ. 
% %
% It is exactly because of this that the final approximation, namely, $\aprxtgtEX$ in Figure~\ref{fig:ambientIntel-system}, will indeed preserve that ``branching" as it does provide useful extra information---in terms of future requests---that helps recover realization.
% 
% Observe also the non-determinism of action $\aWeb$ in full enacted state $s_3$. See that if the game device $\B_G$ happens to evolve to $a_3$ (i.e., enacted system state $s_7$), then a dead-end situation will be reached.
% %%
% This implies that such request-delegation may not be viable and hence all dashed elements will be removed by the $\OptApprox$ algorithm, including the potential transition to ``safe" enacted state $s_8$, as there is no guarantee the whole system will indeed evolve such state. This is why such action will not be accounted in $\aprxtgtEX$.
% \end{example}
% 


Termination of the $\OptApprox$ algorithm is trivially guaranteed, since in the worst case it will remove all  states and transitions. 
%%
More importantly, upon termination, it returns an optimal target approximation.




\begin{theorem}\label{th:soundness}
Algorithm $\OptApprox(\S,\T)$ always terminates and returns an optimal target approximation of target behavior $\T$ on available system $\S$.
% 
% \begin{Proofsk}
% The proof amounts to showing that \myi the target returned by $\OptApprox(\S,\T)$ approximates $\T$; and \myii if there is an approximation ${\aprxtgt}$ of $\T$ such that $\OptApprox(\S,\T) \!\! \preceq \!\! {\aprxtgt}$, then $\OptApprox(\S,\T) \!\! \cong \!\! \aprxtgt$. 
% %%
% %Each state in $\E_{\tup{\S,\T}}$ embeds a target state and transitions from a $\E_{\tup{\S,\T}}$ state are constrained by the allowed actions from the embedded target state. 
% 
% From the definition of $\E_{\tup{\S,\T}}$, it follows that the target $\T$ simulates the full enacted system, i.e.,  $\E_{\tup{\S,\T}} \preceq \T$.
% %%
% Consider target module $\aprxtgt$ after step 8.
% %%
% As Algorithm~\ref{algo:optimalTargetApprox} does not add any new states or transitions to $\E_{\tup{\S,\T}}$, and step 8 merely involves projecting out the index label in transitions, it follows that $\aprxtgt \preceq \T$. Moreover, because $\aprxtgt \cong (\aprxtgt/{\cong_{\aprxtgt}})$, $\OptApprox(\S,\T) \preceq \T$ applies.
% %%
% Furthermore, it is not difficult to see that $\aprxtgt$ represents a fully realizable problem instance---the resulting behavior is non-blocking and each transition has the behavior index to which the target transition can be safety delegated to. 
% %%
% It follows then that $\aprxtgt$ and $\OptApprox({\S,\T})$ have exact composition on $\S$, and therefore are approximations of $\T$.
% 
% 
% For the second part, let $\T'$ be an approximation such that $\OptApprox({\S,\T}) \preceq \T'$.
% %
% Assume $\T'$ is not simulated by $\OptApprox({\S,\T})$.
% %%
% Since  $\E_{\tup{\S,\T}}$ captures all possible evolutions of $\T$ on system $\S$, $\T' \preceq \T$, and $\T'$ has an exact composition, it follows that $\T' \preceq \E_{\tup{\S,\T}}$.
% %%
% Then, in some iteration, the $\OptApprox$ algorithm removed the transitions from $\E_{\tup{\S,\T}}$ that resulted in $\OptApprox({\S,\T})$ not simulating $\T'$.
% %%
% However, only transitions that may lead to dead-end states are deleted.
% %  (i.e., situations where no available behavior can be delegated a legal request).
% %
% Since, by assumption, $\T'  \not \preceq \OptApprox({\S,\T})$, then some of such requests are still represented in $\T'$, and hence, target $\T'$ may lead the system into a dead-end.
% %%
% However, this is a contradiction with the fact that $\T'$ has an exact composition---every trace can be realized and hence no dead-ends can be reached.
% %
% \end{Proofsk}
\end{theorem}


Due to Theorem~\ref{theo:optaprox_solvable} and the compression step, when an exact composition does exist, \OptApprox\ may output a smaller---though equivalent---target behavior than the original one (in fact, it will never be larger).
%%
In terms of computational complexity, it is not hard to see that the problem of deciding whether a given target behavior is an optimal approximation for another target in a system is EXPTIME-complete. First, the $\OptApprox$ algorithm runs in polynomial time on the size of the full system behavior $\E_{\tup{\S,\T}}$, which is exponential on the number of available behaviors, and computing the bisimulation quotient can be done in PTIME~\cite{ModelCheckingBaier:2008}.
%%
Hardness follows trivially from the fact that target approximation subsumes the classical behavior composition problem: to check whether a behavior composition problem has an exact composition, one can compute the optimal target approximation and then check bisimulation with the original target (which can be done in polynomial time).


